Smooth Non-Stationary Bandits

In many applications of online decision making, the environment is non-stationary and it is therefore crucial to use bandit algorithms that handle changes. Most existing approaches are designed to protect against non-smooth changes, constrained only by total variation or Lipschitzness over time. However, in practice, environments often change {\em smoothly}, so such algorithms may incur higher-than-necessary regret. We study a non-stationary bandits problem where each arm's mean reward sequence can be embedded into a $\beta$-H\"older function, i.e., a function that is $(\beta-1)$-times Lipschitz-continuously differentiable. The non-stationarity becomes more smooth as $\beta$ increases. When $\beta=1$, this corresponds to the non-smooth regime, where \cite{besbes2014stochastic} established a minimax regret of $\tilde \Theta(T^{2/3})$. We show the first separation between the smooth (i.e., $\beta\ge 2$) and non-smooth (i.e., $\beta=1$) regimes by presenting a policy with $\tilde O(k^{4/5} T^{3/5})$ regret on any $k$-armed, $2$-H\"older instance. We complement this result by showing that the minimax regret on the $\beta$-H\"older family of instances is $\Omega(T^{(\beta+1)/(2\beta+1)})$ for any integer $\beta\ge 1$. This matches our upper bound for $\beta=2$ up to logarithmic factors. Furthermore, we validated the effectiveness of our policy through a comprehensive numerical study using real-world click-through rate data.

==> beta=1.tex <==
Before delving deep into our focus, the $\beta=2$ case, we analyze the $\beta=1$ case as a warm-up.
We will show a stronger statement than Theorem \ref{thm:be_beta1}.

\begin{proposition}
\label{prop:ub_beta=1}
\Sps\ $6\Delta T\log T \le B^2$. Then \[\mathrm{Reg}\lb(\mathrm{BE}(\Delta, B),\Sigma_1(1,L)\rb) \leq \Delta^{-1}\cdot (1 + L\Delta^2 T + B).\]
\end{proposition}

We then obtain Theorem \ref{thm:be_beta1} by selecting 
\[\Delta = L^{-2/3} T^{-1/3} \log^{1/3} T \text{ and } B=L^{-1/3} T^{1/3} \log^{2/3} T.\]

At a high level, on each epoch the \func\ $\mu$ either (i) is always positive, (ii) is always negative or (iii) has a unique crossing, i.e., $\mu(x)=0$ for some $x$.  
We will bound the regret for these three types of epochs, referred to as {\it positive}, {\it negative} and {\it crossing} epochs, in Lemma \ref{lem:no_crossing>0},
Lemma \ref{lem:no_crossing<0} and 
Lemma \ref{lem:regret_crossing_beta=1} \resp, and then combine them to complete the proof.

% By our construction, the BE \alg\ will select arm $0$, and consequently there is no blindzone regret in this epoch.
% \begin{lemma}
% \Sps\ $r(t) \leq 0$ for all $t\in [0, s]$  for some $s>0$, and $|\frac 1{sT}\sum_{t=1}^{sT} \mu\lb(\frac tT\rb)| \ge T^{-2/5}$.
% Then, whp we have $\sum_{t=1}^{sT} Y_t < 0.$ 
% \end{lemma}
% \begin{proof}
%     I believe this follows directly from Hoeffding.
% \end{proof}
% As a direct consequence, we have the following.

We first consider a positive epoch $i$. 
In this case, the optimal arm is arm $1$, which coincides with the choice of the BE policy before the epoch's stopping rule is triggered.
Thus, there is no regret in this epoch before time $t_i + S_i$.
This can be formally shown by rephrasing Wald's classical identity as follows. 
Recall that $(Z_1^t)$ are the rewards of arm $1$.
% To formalize this idea, we will first 
% We will show that the event $S_i =\Delta T$ is unlikely to occur.
% Thus, regret is incurred only when the stopping rule is triggered before the end of the epoch, i.e. $S_i < \Delta T$.

% We need the following, which follows directly from Wald's stopping time theorem, is useful for both cases.

\begin{lemma}[Wald's Identity, Rephrased]\label{lem:wald}  For any epoch $i$, we have 
$\ho{E}\lb[\sum_{t=t_i}^{t_i + S_i} Z_1^t\rb] =\ho{E}\lb[\sum_{t=t_i}^{t_i + S_i }r(t)\rb]$.
\end{lemma}

As a result, we only need to bound the regret incurred after $t_i + S_i$. 
We will do this by bounding the \prb\  that the budget is ever run out, i.e., $S_i < \Delta T$, as detailed in the next lemma. 
% We formalize this idea in the following.
Recall that $R_t = \max\{0, r(t)\} - Z_{A_t}^t$ is the regret in round $t$.

\begin{lemma}[Regret on Positive Epochs]\label{lem:no_crossing>0}
\Sps\ $\mu(x) > 0$ for $x \in [x_i, x_{i+1}]$.
Then, whenever $B^2 \ge 6 \Delta T \cdot \log T$, the regret of $\mathrm{BE}(B,\Delta)$
on epoch $i$ \sats\ $\ho{E}\lb[\sum_{t=t_i}^{t_{i+1}} R_t\rb] \le 1$.
\end{lemma}

The above essentially follows from the definition of the clean event. 
When $\cal C$ occurs, the cumulative reward up to the first $s$ rounds in this epoch lies within an interval of width $w(s) \lesssim \sqrt s$ of the mean, which is positive.\footnote{{\new When illustrating high level ideas, we use $A\lesssim B$ to denote $A = \Tilde O(B)$.}} 
Further, by the \assu\ that $B\gtrsim \sqrt{\Delta T}$ we have $w(s)\le B$ whenever $s\le \Delta T$.
We defer the proof to Appendix \ref{apdx:positive_epoch}

Now we turn to the negative epochs.

\begin{lemma}[Regret on Negative Epochs]\label{lem:no_crossing<0}
If $\mu(t) < 0$ for  $x\in [x_i, x_{i+1}]$, then the regret on epoch $i$ \sats\  $\ho{E}\lb[\sum_{t=t_i}^{t_{i+1}} R_t\rb] \leq B+1$.
\end{lemma}

We defer the details to Appendix \ref{apdx:negative_epoch}.
The above follows from 
the definition of the stopping time $S_i$. 
In fact, if the process never stops until the end of epoch, then the cumulative reward is above $-B$. 
If it does stop at some $s<\Delta T$, then the cumulative reward is {\bf just} below $-B$, and hence above $-(B+1)$ since  $|Z_1^t|\le 1$. 

Finally we consider crossing epochs. The following essentially follows from the Lipschitzness of $\mu$.

\begin{lemma}[Regret on Crossing Epochs]\label{lem:regret_crossing_beta=1}
Let $j$ be a crossing epoch, i.e.,  $\mu(\tilde x) =0$ for some $\tilde x\in [x_j, x_{j+1}]$.
Then, the regret in this  epoch \sats\ $\ho{E}\lb[\sum_{t=t_j}^{t=t_{j+1}} R_t\rb] \le 2L \Delta^2 T$.
\end{lemma}
\begin{proof}
By Lipschitzness of $\mu$, we have $|\mu(x)| = |\mu(x)-\mu(\tilde x)| \le  L\Delta$  whenever $x_j\le  x\le x_{j+1}$. 
In the original time scale, this means $|r(t)|\le L\Delta$ whenever $t_j \le t\le t_{j+1}$, and hence 
\[\sum_{t=t_j}^{t_{j+1}} |r(t)| \le \Delta T  \cdot L\Delta = L\Delta^2 T.\]
To connect the above with the regret, observe that
\begin{align*}
\ho{E}\lb[\sum_{t=t_j}^{t_{j+1}} R_t\rb] &= \ho{E} \lb[ \sum_{t=t_j}^{t_{j+1}} \lb(\max\{0, r(t)\} - Y_t\rb)\rb] \\
&\leq \sum_{t=t_j}^{t_{j+1}}  \big|r(t)\big|   - \ho{E}\lb[\sum_{t=t_j}^{t_{j+1}} Z_{A_t}^t\rb].
\end{align*}
Moreover, for each $t$ we have $|\ho{E} [Z_{A_t}^t]| \leq |r(t)|$, so  
\[\ho{E} \lb[\sum_{t=t_j}^{t_{j+1}}  R_t\rb] \le 2 \sum_{t=t_j}^{t_{j+1}}  \big|r(t)\big| \le 2L \Delta^2 T.\]
\end{proof}

We are now ready to show the $\tilde O(T^{2/3})$ upper bound. 
To suppress notations, we will subsequently  write  $R[i]=\ho{E}\lb[\sum_{t=t_i}^{t_{i+1}} R_t\rb]$ as the regret on epoch $i$.

{\bf Proof of Proposition \ref{prop:ub_beta=1}.}
Let $J_+, J_-, J_{\mathrm{x}} \subseteq \{1,\dots,\Delta^{-1}\}$ be the subsets of positive, negative and crossing epochs. 
Note that  $J_+ \cup J_- \cup J_{\mathrm{x}} = 
\{1,\dots,\Delta^{-1}\}$, so the total regret can be decomposed as 
\begin{align}\label{eqn:011323}
\sum_{i=1}^{1/\Delta} R[i] = \sum_{i\in J_-} R[i]  +  \sum_{i\in J_+} R[i]  +  \sum_{i\in J_\mathrm{x}} R[i].
\end{align}
By Lemma \ref{lem:no_crossing>0}, Lemma \ref{lem:no_crossing<0} and Lemma \ref{lem:regret_crossing_beta=1}, whenever $6\Delta T\log T \le B^2$, we have 
\begin{align*}
\eqref{eqn:011323} &< |J_+| \cdot 1 +  |J_-| \cdot (B+1) + |J_\mathrm{x}| \cdot 2 L\Delta^2 T \\
&\le \Delta^{-1}\cdot (1 + B + L\Delta^2 T). &\quad \qed
\end{align*}

==> cone_alg.tex <==
As a warm up, we start with the case where $\beta= 1$, i.e., assuming $\mu$ to be $L$-Lipschitz for some constant $L>0$.
% Let $\mathcal{F}$ be the family of all reward functions that are 1-Hölder in $t$, then BGZ’s  algorithm
Recall from \cite{besbes2015non} that a Multiplicative Weight \alg\ achieves 
$O(V^{1/3}T^{2/3})$ for any \env\ $\mu$ with {\it total variation} $V$, i.e. 
$V = \sum_{t=1}^T |R(t) - R(t+1)|.$

This immediately implies an $O(L^{1/3} T^{2/3})$ upper bound for $\beta=1$. 
Indeed, observe that if $\mu:[0,1] \to [-1,1]$ is $L$-Lipschitz, then its total variation can be bounded as 
\begin{align*}
V &= \sum_t |R(t)-R(t+1)| \\
&= \sum_t \Big|\mu\lb(\frac tT\rb)-\mu\lb(\frac {t+1}T\rb)\Big| \\
&\leq \sum_t L\cdot \Big|\frac tT-\frac {t+1}T\Big| = L,
\end{align*}
and the claim follows.

To gain insight for general $\beta$, in this section we present an alternate \alg\ that also achieves this regret but via a completely different approach: local polynomial regression.
At a high level, \hw{describe the high level idea} at the end $t$ of an epoch, if the reward estimation $P(t) > 0$, choose arm $1$ in the next $\Delta T$ rounds, else build a confidence cone using only the data from this epoch, choose arm $0$ until the cone contains $0$. The formal definitions of epoch and confidence cone are given below.

\begin{definition}[Exploration epoch for $\beta=1$, ``one-arm"]
An exploration epoch (abbr. epoch) is a contiguous $T^{1/3}$ number of rounds where we always pick arm $1$.     
\end{definition}

\begin{definition}[Confidence cone for $\beta=1$]
Without loss of generality let $[0, \Delta]$ be an epoch, $\Delta = T^{-1/3}$. Consider $x_0 = \Delta - h$ where $h = \Theta(\Delta)$. 
Let $P(x_0)$ be the estimate of $R(x_0)$ returned by the local polynomial regression estimator.
Let $P(t)$ be a degree-$0$ polynomial (i.e., a constant) “prediction” based on the $0$-th derivative of $P$ at $x_0$, i.e., $P(x_0)$. Formally, $P(x_0 + t) := P(x_0)$ for all $t$.
Then the ``confidence cone" is given by 
$U(x_0 + t) = P(x_0 + t) + Lt$	and	$L(x_0 + t) = P(x_0 + t) - Lt$.
\end{definition}
\qx{It seems that we have duplicate definitions of the confidence cone. Do we need to remove this one?}

We formally define the Confidence Cone (CC) 
\Alg\ in Algorithm~xxx.
With some foresight, we choose $\Delta= T^{-1/3}$. \demo{rigorify the pseudocode}
\qx{Not sure whether to use the orginal time scale or the normalized time scale in the pseudocode. I'll also make the notations consistent.}

\bitem 
\item In the first $\Delta$ time, perform local polynomial regression with bandwidth $h\sim \Delta$ to obtain an estimated reward \func\ $\hat R(x)$
\item Build a (blue) cone, see Figure~\ref{fig:beta_1}
\item Before the cone hits 0, choose arm 1 if $\hat R(x-h)\geq 0$ and arm 0 \ow.
\item When the cone hits 0, choose arm 1 for the next $\Delta$ time (such an interval of length  $\Delta$ is called an ``epoch''), repeat. \su{in a pseudo-code, should not say ``repeat''. Instead, use a while loop}
\eitem 

\begin{algorithm}[tb]
   \caption{Smooth Non-stationary Stochastic Bandit}
   \label{alg:beta_1}
\begin{algorithmic}
   \STATE {\bfseries Input:}
   \STATE Initialize $t=0$
   \WHILE{$t\leq T$}
    \STATE Pull arm $1$ in the epoch $[t,t+\Delta T]$ and collect reward \\
    \STATE Perform local polynomial regression with bandwidth $h=\Theta(\Delta)$ to obtain an estimated reward \func\ $\hat R$ on $[t/T, t/T+\Delta]$ \\
    \STATE Let $x=t/T+\Delta-h$
    \STATE Set confidence interval upper bound $U(x)=\hat R(x)$ \\
    \STATE Set confident interval lower bound $L(x)=\hat R(x)$
    \WHILE{confidence interval $[L(x), U(x)]$ does not contain 0}
        \IF{$\hat R(x)\geq0$}
            \STATE Choose arm $1$
        \ELSE
            \STATE Choose arm $0$
        \ENDIF
        \STATE Update $U(x)$ with $U(x)+LT^{-1}$
        \STATE Update $L(x)$ with $L(x)+LT^{-1}$
        \STATE Update $x$ with $x+T^{-1}$
    \ENDWHILE
    \STATE Update $t$ with $x\cdot T$
   \ENDWHILE
\end{algorithmic}
\end{algorithm}

\begin{figure}
\centering    \includegraphics[width=\linewidth]{figures/beta_1.png}
    \caption{Confidence Cone Algorithm $\beta=1$ \su{update this picture, I want the red cone to be higher than the blue cone}}
    \label{fig:beta_1}
\end{figure}


We show that the CC \alg\ achieves the same $T^{2/3}$ regret.
\begin{theorem}[Regret of Confidence Cone \Alg]\label{thm:cc}
The Confidence Cone \Alg\ $\ho{A}$ \sats\ $\mathrm{Reg}\lb(\ho{A}, \Sigma(1,L)\rb) = \tilde {O}_L(T^{2/3})$.
\end{theorem}


\begin{definition}[Clean Event]
Define the {\it clean event} $\cal C$ to be xxx \su{tbd}
\end{definition}

Observe that there are at most $1/\Delta = T^{1/3}$ epochs.
In \parti, this means we only need to consider finite number of $i$'s, rendering the exchangeablility of summations easier to handle.

\begin{definition}[Epoch Starting Time $T_i$]
For each $i=1,...,T^{1/3}$,
denote by $T_i$ the starting time of the $i$-th epoch, if it exists; 
\ow, define $T_i = T$.
\end{definition}
Consequently, $T_i + \Delta$ is the ending time of the $i$-th epoch. 

In our analysis, we will consider another closely-related notion of stopping time $S_i$. 
Essentially, this is the hitting time of the confidence cone if there were no noise in the estimation.  
% Imagine translating the  the confidence cone vertically so that it contains $(T_i, \mu(T_i))$, $S_i$ is essentially the time when this cone hits the t-axis. 
\begin{definition}[Noiseless Cone]
Fix any integer $i\geq 1$.
Define the $i$-th {\it noiseless confidence cone} to be the set 
\[K_i = \{(T_i + t,y): t\geq 0,\ K^-_i (t)\leq y\leq K^+_i (t)\}\] 
where
$K^\pm_i(T_i + t) = \mu(T_i) \pm Lt$. 
Correspondingly, the $i$-th {\it noiseless hitting time} is defined as $S_i = T_i + \frac 1L \cdot \mu(T_i)$.
\end{definition}

We will use the following nice property of $S_i$.
By definition of 1-Hölder, the graph of $\mu$ lies within the cone $K$, and hence will not hit $0$ prior to $S_i$.
Consequently, selecting arm 0 incurs {\it no} regret in $[T_i, S_{i+1}]$.

\begin{lemma}[No Regret Before $S_{i+1}$]\label{lem:no_regret_by_Si}
For any integer $i$, we have $\sum_{t=T_i+\Delta}^{S_{i+1}} R_t=0$ a.s.
\end{lemma} 
\begin{proof}
\su{pretty obvious}
\end{proof}
 
\begin{lemma}[Bounding the Extrapolation Error]\label{lem:121322}
If $\cal C$ occurs, then
for any $t\in [S_{i+1}, T_{i+1}+\Delta]$, we have
$|\mu(t)| \leq 2|\mu(t_i)| + T^{-1/3} + L\Delta$. 
\end{lemma}
\qx{Need to define $\mathcal{C}$.}
\begin{proof} Use Lipschitzness and concentration.

Step 1: show  $|T_{i+1} - S_{i+1}| \leq \frac 1L \cdot T^{-1/3}$.

Step 2: Show
$|\mu(S_{i+1})| \leq 2|\mu(T_i)| + T^{-1/3}$
\end{proof}


\begin{lemma}[Upper Bound on the Amortized Regret]
\Sps\ the $\cal C$ occurs. 
Then for any integer $i\geq 1$, the total regret in the $i$-th \ac\ is $O\lb(2L \cdot \lb(\Delta + \frac 1L T^{-1/3}\rb)\rb)$.
\end{lemma}
\begin{proof}
We start with bounding the  regret in terms of $|\mu|$.
By Lemma \ref{lem:no_regret_by_Si}, \begin{align}\label{eqn:regret_i}
\sum_{t=T_i+\Delta}^{T_{i+1}+\Delta} R_t 
=\sum_{t=S_{i+1}+1}^{T_{i+1}+\Delta} R_t
\leq\sum_{t=S_{i+1}+1}^{T_{i+1}+\Delta}|\mu(t)|.
\end{align}
By Lemma \ref{lem:121322}, we have
\begin{align*}
\eqref{eqn:regret_i} &\leq \sum_{t=S_{i+1} + 1} ^{T_{i+1} + \Delta} \lb(2|\mu(T_i)| + T^{-1/3} + L\Delta\rb) \\
&= \lb(\Delta + T_{i+1}- S_{i+1}\rb)\cdot \lb(2|\mu(T_i)| + T^{-1/3} + L\Delta\rb)
\end{align*}     
Note that the length of the \ac\ is bounded by 
\begin{align*}
\Delta + T_{i+1} - T_i &= (S_{i+1} - T_i) + (T_{i+1} - S_{i+1}) + \Delta \\
&= \frac 1L \cdot \mu(T_i) + \Delta + \frac 1L T^{-1/3}
\end{align*}
Dividing, we can bound the amortized regret by 
\begin{align*}
AR &\leq \frac{\lb(\Delta + T_{i+1}- S_{i+1}\rb)\cdot \lb(2|\mu(T_i)| + T^{-1/3} + L\Delta\rb)}{\frac 1L \cdot \mu(T_i) + \Delta + \frac 1L T^{-1/3}} \\
&\leq 2L \cdot \lb(\Delta + \frac 1L T^{-1/3}\rb),
\end{align*}
and the proof is complete.
\end{proof}

Using this lemma, we can obtain the following upper bound on the total regret by partitioning $[0,1]$ into \ac s.  
The main technical challenge in the proof lies in handling the randomness of the epochs' starting time. 

\noindent{\bf Proof of Theorem \ref{thm:cc}.}
The total regret is
\[\ho{E}\lb[\sum_t R_t\rb] = \ho{E}\lb[\sum_{i= 1}^{1/\Delta} \sum_{t=T_i}^{T_{i+1}} R_t\rb]\]
\qed
